Any Deep ReLU Network is Shallow

We constructively prove that every deep ReLU network can be rewritten as a functionally identical three-layer network with weights valued in the extended reals. Based on this proof, we provide an algorithm that, given a deep ReLU network, finds the explicit weights of the corresponding shallow network. The resulting shallow network is transparent and used to generate explanations of the model s behaviour.

==> content-trial.tex <==
\begin{abstract}
We constructively prove that every deep ReLU network can be rewritten as a functionally identical three-layer network with weights valued in the extended Reals. Based on this proof, we provide an algorithm that, given a deep ReLU network, finds the explicit weights of the corresponding shallow network. The resulting shallow network is transparent and used to generate explanations of the model's behaviour. 
%We give a constructive proof that every deep ReLU network can be rewrite exactly as a three-layer network with weights valued in the extended Reals. This is used to produce interpretable networks whose behaviour is fully understood. We provide an algorithm to obtain the shallow network. 
    % We prove that any ReLU neural network can be implemented as a shallow network of depth 3. Our proof is constructive. However, since we use inf weights, the resulting shallow network can not be fine-tuned. We investigate time to compute the shallow network and how it can be used for explainability of the original network.
\end{abstract}

\section{Introduction}

Deep learning systems are leveraged for their flexibility and performance to solve real world tasks efficiently; yet, their complexity warrants in-depth analysis of their behaviour and underlying mechanisms to provide safety and soundness guarantees. 
% With growing adoption of neural networks, in Artificial Intelligence (A.I.) systems, 
% interpreting their behaviour is increasingly a priority. Deep learning systems are interwoven with human decision-making, which leverages the flexibility and performance of these models to solve real world tasks efficiently; yet, their complexity warrants an in-depth analysis of their behaviour and underlying mechanisms to provide safety and soundness guarantees. 
%Efforts in Explainable Artificial Intelligence (XAI) \citep{Samek2021}, mechanistic interpretability \citep{Chris Olah}, and deep learning theory \citep{PDLT-2022} all aim to make neural networks more explainable, interpretable and transparent.
% If we want to cite papers in the field of "inductive biases"/"the science of deep learning" we can cite the Lottery Ticket Hypothesis and Grokking
In light of this, we present a method to convert black-box neural networks into functionally identical shallow white-box networks. Our contributions are: 
% the fact that networks can be flattened may aid our understanding of inductive biases that are more favourable for specific network depth-width ratios. 
% the contributions
\begin{enumerate}[topsep=0pt]
    \item A constructive proof of the existence of functionally identical shallow network (three hidden layers) with weights in the extended Reals for every deep ReLU network, (Section \ref{sec:shallow-network-theorem}); 
    \item An algorithm to find the values of these weights given a trained network (Section \ref{sec:implementation}), which relies on searching the space of possible neuron activations through heuristics that we prove to be exhaustive; and 
    \item Explainability improvements that arise from the shallow network construction (Section \ref{sec:interpretability}) including fast SHAP Values.
\end{enumerate}

Our constructive proof permits explicit specification of the weights, thus enabling us to compute the shallow network algorithmically. 
The code for replicating our experiments is provided in the Appendix. 
% CHAT GPT 4 

Existing literature on explainability in deep neural networks predominantly focuses on local interpretation of ReLU networks \citep{Samek2021}. These advances rely on the exact representation of ReLU networks as a decomposition of local linear models. 
\citet{sudjianto2020unwrapping} find explicit weights of local linear models for ReLU networks as a function of the weights. Other works compute local approximations of neural networks as explanations \citep{Dong2021}, or use them to analyse phenomena such as dying neurons 
\citep{Jiang2022}.
Conversely, \citet{He2021} proves that every piecewise linear function on a bounded domain can be realised as a ReLU network of a given depth, provided as a function of the linear regions.  

 This study extends these findings by enhancing the theoretical understanding of neural networks and establishing a firm connection between linear programming and ReLU activation patterns. Consequently, our work advances global interpretability of neural networks and provides effective heuristics for exploring the extensive search space of activation patterns. 
% This development is anticipated to positively influence our ability to modify, train, verify networks, and assess their fairness. 
%CHAT GPT 4
%Our work extends existing results by furthering the theoretical understanding of neural networks. It also explicitly computes local regions and tightens the connection between linear programming and ReLU activation patterns. This enables global interpretability of neural networks, while providing heuristics to navigate the vast search space of activation patterns. In turn, this has positive repercussions on our ability to modify, train, verify networks, and assess their fairness. 

\section{Background}\label{sec:background}
We restrict our analysis to architectures which are feed-forward neural networks; in particular, those whose activation function for each layer is the rectifier linear unit (ReLU). 

\begin{definition}[ReLU Network]
A ReLU network $\mathcal{N} \colon \mathbb{R}^n \rightarrow \mathbb{R}^m$, is a composition of $L \in \mathbb{N}$ hidden layers given by: 
\[ \chi^{(l)} = \sigma( {W^{(l)}} \chi^{(l-1)} + b^{(l)}),\]
where $\sigma$ is an element-wise ReLU activation function, $\sigma(x_i) = \max\{0,x_i\}$. We define $\chi^{(0)} = x$ and the output layer is given by $\mathcal{N}(x) = W^{(L+1)} \chi^{(L)} + b^{(L+1)}$. 
The number of neurons in each layer is given by a vector $\mathbf{N} = [n_1, n_2, \ldots, n_L]$, and all activations are in the positive Reals, i.e. $\chi^{(l)} \in \mathbb{R}^{n_l}_{\geq 0}$ for all $l \in \{1,\ldots,L\} = [L]$.
\end{definition}

Work by \citep{sudjianto2020unwrapping} makes explicit a decomposition of neural networks as piece-wise linear functions. We can describe these functions as linear models that are applied to certain convex regions of the input space. Moreover, these regions partition $\mathbb{R}^n$. We deduce the following function between pairs of networks and prove this is a distance measure. 

\begin{greybox}
\begin{example}
Consider the network given by the weight matrix 
$ W 
= \begin{bmatrix} 1 & 1 \\ 1 & 0  \end{bmatrix}. 
$
Let the input vector be $\begin{bmatrix} x_1 \\ x_2 \end{bmatrix}$. Then, the output of of this network, after applying the ReLU activation function, is
$\begin{bmatrix}
y_1 \\
y_2
\end{bmatrix} =
\text{ReLU} \left( \begin{bmatrix}
1 & 1 \\
0 & 1
\end{bmatrix}
\begin{bmatrix}
x_1 \\
x_2
\end{bmatrix} \right) =
\text{ReLU} \left( \begin{bmatrix}
x_1 + x_2 \\
x_2
\end{bmatrix} \right) =
\begin{bmatrix}
\max(0, x_1 + x_2) \\
\max(0, x_2)
\end{bmatrix}.
$

This gives us a partition of the input space $\mathbb{R}^2$. The boundaries are determined by the points where the vector output of the linear transformation has entries equal to zero. 
% \begin{figure}[H]
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%     \includegraphics[width=0.4\textwidth]{figures/sketch-diagonal-new.png}
%     \captionsetup{labelformat=empty}
%     \caption{}
%     \label{fig:}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/sketch-y-big.png}
%     \captionsetup{labelformat=empty}
%     \caption{}
%     \label{fig:}
% \end{subfigure}
% \captionsetup{labelformat=empty}
% \caption{}
% \end{figure}
\vspace{-1.5cm}
% Then, the four parts are given by: \\
% $\omega_1 = \{(x_1,x_2) : x_1 + x_2 > 0, x_2 > 0 \}$, \\ 
% $\omega_2 = \{(x_1,x_2) : x_1 + x_2 \leq 0, x_2 > 0 \}$, \\
% $\omega_3 = \{(x_1,x_2) : x_1 + x_2 > 0, x_2 \leq 0 \}$, \\
% $\omega_4 = \{(x_1,x_2) : x_1 + x_2 \leq 0, x_2 \leq 0 \}$, \\
% \begin{wrapfigure}{R}{0.5\textwidth}
%     \includegraphics[width=0.48\textwidth]{figures/sketch-4-parts-omegas.png}
% \captionsetup{labelformat=empty}
% \caption{}
% \end{wrapfigure}
% such that $\Omega = \{\omega_1, \omega_2,\omega_3,\omega_4\}$ covers the input space.

Then, the four parts are given by: \\
\[\omega_1 = \{(x_1,x_2) : x_1 + x_2 > 0, x_2 > 0 \},  
\omega_2 = \{(x_1,x_2) : x_1 + x_2 \leq 0, x_2 > 0 \}, \]
\[ \omega_3 = \{(x_1,x_2) : x_1 + x_2 > 0, x_2 \leq 0 \},
\omega_4 = \{(x_1,x_2) : x_1 + x_2 \leq 0, x_2 \leq 0 \}, \]
such that $\Omega = \{\omega_1, \omega_2,\omega_3,\omega_4\}$ covers the input space.
\begin{figure}[H]
    \begin{center}
    \includegraphics[width=0.28\textwidth]{figures/sketch-4-parts-no-background-new.png}
    \end{center}
% \captionsetup{labelformat=empty}
\end{figure}
\end{example}
\end{greybox}

\begin{proposition}\label{prop:network-to-partition}[ \citet{sudjianto2020unwrapping}]
For a ReLU network $\mathcal{N} \colon \mathbb{R}^n \rightarrow \mathbb{R}^m$ there is a finite partition $\Omega$ of $\mathbb{R}^n$ of cardinality $\# \Omega = p$ such that for each part $\omega \in \Omega$ there exists a piece-wise linear function $f\colon \mathbb{R}^n \rightarrow \mathbb{R}^m$ such that its restriction on $\omega$, denoted $f|_\omega$ can be described by a linear function: 
\[f|_\omega (x) = \alpha_\omega^T x + \beta_\omega.\]
Moreover, each part is a convex polytope, given by the intersection of a collection of half-spaces.
We write the minimum set of half-space conditions that can be used to specify the entire partition as $H_1,\ldots,H_k$, where each $H_i$ is given by the set of all $x \in \mathbb{R}^n$ such that: 
\[ h_{i,1} x_1 + h_{i,2} x_2 + \ldots + h_{i,n} x_n  > c_i.\]
\end{proposition}

To represent the decomposition and linear models, it is useful to characterise the states of a neural network by looking at which neurons are active and inactive in all layers. 
% For all $i \in [n_l]$, we can encode the activation state of each neuron in an \textit{activation vector}. The collection of all activation vectors for all layers is called the \textit{activation pattern} of the neural network. 

\begin{definition}[\textbf{Activation Pattern}] For a given ReLU network $\mathcal{N} \colon \mathbb{R}^n \rightarrow \mathbb{R}^m$ with neuron dimensionality vector $\mathbf{N} = [n_1,\ldots,n_L]$, the activation pattern at a point $x \in \mathbb{R}^n$ is a collection of vectors $P = \{P^{(1)},\ldots, P^{(L)}\}$, with $P^{(l)} \in \{0,1\}^{n_l}$ for each $l \in [L]$, such that for all $i \in [n_l]$, 
\[P^{(l)}_i = 1 \iff \chi^{(l)}_i > 0 . \]
\end{definition}
% We say that a neuron $\chi^{(l)}_{i}$ is active whenever it is different from zero. 

\section{Finding a Shallow Network for a given Piecewise Linear Function} \label{sec:shallow-network-theorem}

Figure \ref{fig:conversion} illustrates the intuition that a network can be fully characterized by 1) the partition; and 2) a linear model for each item in the partition. This suggests that we can convert any deep network into a shallow one. We will now formalize and prove this intuition.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/construction-our-own-partition.png}
    \caption{A high-level representation of the conversion of a deep ReLU network (left) using a decomposition of the input space into regions that each have their own linear model (middle) to a shallow ReLU network (right).}
    \label{fig:conversion}
\end{figure}

% https://q.uiver.app/?q=WzAsMyxbMiwwLCJcXG1hdGhiYntSfV5uIFxcdGltZXMgXFxwcm9kX3tJfVxcezAsMVxcfSJdLFswLDAsIlxcbWF0aGJie1J9Xm4iXSxbNCwwLCJcXG1hdGhiYntSfV5tIl0sWzEsMCwiaWQgXFx0aW1lcyBhY3QiXSxbMCwyLCJcXHRleHR7ZXZhbH0iXSxbMSwyLCJcXG1hdGhjYWx7Tn0iLDAseyJjdXJ2ZSI6LTV9XV0=
% \[\begin{tikzcd}
% 	{\mathbb{R}^n} && {\mathbb{R}^n \times \prod_{I}\{0,1\}} && {\mathbb{R}^m}
% 	\arrow["{\texttt{id} \times \texttt{act}_\mathcal{N}}", from=1-1, to=1-3]
% 	\arrow["{\texttt{eval}}", from=1-3, to=1-5]
% 	\arrow["{\mathcal{N}}", curve={height=-30pt}, from=1-1, to=1-5]
% \end{tikzcd}\]% Related papers on mode connectivity
% A network can be rewritten as two functions, one that associates the input to a region in the input partition via its activation pattern, which we call $\texttt{act}$. The range is a subset of all possible activation patterns $\prod_{I}\{0,1\}$, where $I = \oplus^{L}_{l = 1} [n_l]$ is an indexing set defined through the direct sum operator. To each of these activation patterns, we associate a linear model through the function $\texttt{eval}$, which takes the $\mathbb{R}^n$ input and activation pattern and applies the local linear model at that point. 

\begin{theorem}\label{theorem:main-shallow}
For every ReLU network $\mathcal{N} \colon \mathbb{R}^n \rightarrow \mathbb{R}^m$, there exists a shallow neural network $\mathcal{S} \colon \mathbb{R}^n \rightarrow \mathbb{R}^m$ of depth $L = 3$, with weights in the extended Reals $\bar{\mathbb{R}} = \mathbb{R} \cup \{\infty\}$ such that for all $x \in \mathbb{R}^n$, the following holds: 
\[\mathcal{N}(x) = \mathcal{S}(x). \]
\end{theorem}

\begin{proof}

Our strategy will be to build a first layer that encodes the linear models and the half-spaces that span the partition. 
We will use the weights that encode the half-spaces to, in the last layer, select the correct linear model out of the list of linear models. 
See Figure \ref{fig:schematic-rep-of-proof} for an overview of the components of the shallow network.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/Picture 1.pdf}
    \caption{A schematic representation of the shallow network. }
    \label{fig:schematic-rep-of-proof}
\end{figure}

Let $(\{f_\omega\}_{\omega \in \Omega}, \Omega)$ be the decomposition that corresponds to $\mathcal{N}$. Label the parts $1,\ldots,p$. Recall that each part is a polytope and we can represent it as the intersection of half-spaces. In particular, let $H_1,\ldots,H_k$ be the the minimum set of half-spaces that specify the partition, where each $H_i$ is given by the set of all $x \in \mathbb{R}^n$ such that: 
\[ h_{i,1} x_1 + h_{i,2} x_2 + \ldots + h_{i,n} x_n  > c_i.\]
Let $\Psi$ be a linear transformation applying all the half-space conditions: 
\begin{align*}
    \Psi(x) = H x + c 
    = \begin{bmatrix} -h_{1,1} & -h_{1,2} & \ldots & -h_{1,n} \\ -h_{2,1} & -h_{2,2} & \ldots & -h_{2,n}\\ \ldots & & & \ldots \\  - h_{k,1} & - h_{k,2} & \ldots & - h_{k,n} \end{bmatrix} \begin{bmatrix} x_1 \\ x_2 \\\ldots \\ x_n \end{bmatrix}+ \begin{bmatrix} c_1 \\ c_2\\  \ldots \\ c_k \end{bmatrix}, 
\end{align*}
where $H$ is a $2k \times n$ matrix. 
Entry-wise this matrix $\Psi(x)$ looks as follows
\[\Psi(x)_{i} = - h_{i,1} \cdot x_1 - h_{i,2} \cdot x_2 -  \ldots - h_{i,n} \cdot x_n + c_{i}.\] 
% Notice that this implies that $ReLU(B(x))$ has a positive entry at $2i-1$ only if $x\in H_i$, and $ReLU(B(x))_{2i} = 0 $ whenever $x \in H_i$. 
Notice that this implies that whenever $x\in H_i$ we have $\text{ReLU}(\Psi(x))_{i} = 0$. 
The \textbf{first layer} is given by: 
\[
\chi^{(1)} = \text{ReLU}( W^{(1)}x +b^{(1)})  =\text{ReLU} \left(\begin{bmatrix}
    I_n \\
    - I_n \\
    H 
\end{bmatrix} x + \begin{bmatrix} 0 \\ 0 \\ c \end{bmatrix} \right),
\]
which is an activation vector of length $2\cdot n + k$.

This transformation develops the building blocks to generate neurons that are only inactive when $x$ is in a certain region: we want to construct a layer that only has an inactive neuron whenever the input is in a particular region. 
In other words, we find a $p \times k$ zero-one matrix $R$ which describes the regions in terms of which boundaries are active. Precisely, we can design $R$ so that $R \cdot \text{ReLU}(\Psi(x))$ has a zero entry at $j$ only when $x \in \mathbb{\omega}_j, j \in \{1,\ldots,p\}$. 
Assume without loss of generality that the  half-space conditions corresponding to region $\omega_j$ are $H_1, \ldots , H_a$. The half-space conditions $H_1, \ldots , H_a$ are satisfied at a point $x$ if and only if $x \in \omega_j$.
We construct $R$ such that at row $j$ it assigns a 1 to entries $1, \ldots, a$, and a 0 to all other entries in that row.  
This leads to the description of the \textbf{second layer}: 
\begin{align*}
\chi^{(2)} 
= \text{ReLU}( W^{(2)} \chi^{(1)} + b^{(2)}) 
&= \text{ReLU} 
\left(\begin{bmatrix} 
I_{n} & 0 & 0 \\ 
 0& I_{n} & 0 \\
 0& 0 & R \end{bmatrix} \chi^{(1)} + \begin{bmatrix}
    0 \\ \vdots  \\ 0
\end{bmatrix} \right) \\
& = \text{ReLU} \left(\begin{bmatrix} \hspace{12pt} \text{ReLU}( x )  \\
\hspace{12pt} \text{ReLU}( - x) \\
R \cdot \text{ReLU}(\Psi(x)) \end{bmatrix} \right), 
\end{align*} 
as an activation vector of length $2 \cdot n + p$.
 
Finally, in the third layer we 1) multiply the input with each of the linear models, and 2) use the indicator function that is only zero at entry $p$ if the input $x$ is in part $p$, to isolate the correct linear model. Without loss of generality, we assume that $m = 1$ so that $\mathcal{N}: \mathbb{R}^n \rightarrow \mathbb{R}$. If the dimension of the output space $m >1$, then we repeat the construction of the last layer $m$ times. 

Let $\Lambda$ be a linear transformation given by: 
\[
\Lambda(x) = \alpha^T x + \beta,
\]
where $\alpha, \beta$ are respectively a $p \times n$ matrix and a $p$-dimensional bias, such that the row $\alpha_i$ and entry $\beta_i$ contain the coefficients of $f_i$. Note that, in this step, if $m > 1$, then the matrix and vector would be $p \cdot m \times n$ and $p \cdot m$ dimensional respectively.

We construct a matrix $ O_{p} = \theta \cdot I_{p}$, where $ \theta = \infty$, such that $\infty \cdot 0 = 0$ and $\infty \cdot a = \infty$ for all $|a| >0, a \in \mathbb{R}$.
Note that Python contains such a constant, denoted by \texttt{inf}. 
We use this matrix so that when we subtract it from a matrix of linear models, the only unaffected linear model will be $f_j$, i.e.
\[\Lambda(x) - O_p \cdot \text{ReLU} (R \cdot \text{ReLU}(\Psi(x))) 
= \begin{bmatrix} - \infty \\ \vdots \\ -\infty \\\Lambda(x)_j \\ - \infty \\ \vdots \\ - \infty \end{bmatrix},\] 
which is a vector of length $p$ for which the only positive entry is given by the linear model at the region $j$ evaluated at $x$. 
Since elements of other regions can lie arbitrarily close to region $\omega_j$, each $R\cdot \text{ReLU} (\Psi(x))$ can be arbitrarily small, and so we can not just choose a very large number instead of infinity. 
This entails our \textbf{third layer} activations are given by:   
\begin{align*}
\chi^{(3)} 
= 
\text{ReLU}(W^{(3)} \chi^{(2)} + b^{(3)}) 
& = \text{ReLU} \left(\begin{bmatrix} \alpha & \alpha  & - O_{p} \\ -\alpha 
& -\alpha  & - O_{p}  \end{bmatrix} \chi^{(2)} + \begin{bmatrix} \beta \\ -\beta \end{bmatrix}\right) \\
& = \text{ReLU} \left( \begin{bmatrix} \alpha & \alpha  & - O_{p} \\ -\alpha & -\alpha  & - O_{p}  \end{bmatrix} \begin{bmatrix} \hspace{12pt} \text{ReLU}(x) \\ \hspace{12pt} \text{ReLU}( - x) \\ R \cdot \text{ReLU}(\Psi(x)) \end{bmatrix} + \begin{bmatrix} \beta \\ -\beta \end{bmatrix}\right) \\
& = \text{ReLU} \left( \begin{bmatrix} \hspace{3.5pt} \Lambda(x)  \hspace{4pt} - O_{p} \cdot \text{ReLU} \left(R \cdot \text{ReLU}(\Psi(x)) \right) \\ -\Lambda(x) - O_{p} \cdot \text{ReLU}\left(R \cdot \text{ReLU}(\Psi(x))\right) \end{bmatrix} \right)
\end{align*}
which is a vector of length $2 p$ with exactly one non-zero entry at either $j$ or $2j$. This non-zero entry is $\Lambda(x)$ at row $j$ (if $\Lambda(x)$ is positive) or $-\Lambda(x)$ at row $2j$ (if $\Lambda(x)$ is negative). 

Lastly we need a weight matrix to project onto $\mathbb{R}^m$. This projection requires $2p$ weights. When we project the $-\Lambda(x)$ value to the output layer, we need to swap the sign. The first $p$ weights of $W^{(4)}$ are 1 and the last $p$ weights are $-1$: 
\[ \mathcal{S}(x) = W^{(4)} \cdot \chi^{(3)}  = \Lambda(x)_j = \mathcal{N}(x).\]

Note that here we assumed $m=1$. In general, the length of $\chi^{(3)}$ is $2 \cdot p \cdot m$, and the number of required projection weights is $2 \cdot p \cdot m$.
\end{proof}

\begin{corollary}
Given a ReLU network $\mathcal{N} \colon \mathbb{R}^n \rightarrow \mathbb{R}^m$, the shallow network $\mathcal{S} \colon \mathbb{R}^n \rightarrow \mathbb{R}^m$ of depth $L = 3$, 
as specified in the proof of Theorem \ref{theorem:main-shallow} has width bounded by \[  \max \{ 2n+k, 2n+p, 2\cdot p \cdot m \}, \]
where $p = \# \Omega$ and $k = \# \{ \text{half space conditions} \}$.
\end{corollary}
Note that \citet{montufar2014number},  \citet{Serra2020}, and \citet{Chen2022}, find progressively tighter bounds for the number of linear regions in ReLU networks as functions of the number of neurons at each layer.
\begin{corollary}
For every continuous piece-wise linear function $f$, there exists a shallow neural network $\mathcal{S}$ of depth $L = 3$ with weights in the extended Reals $\bar{\mathbb{R}} = \mathbb{R} \cup \{\infty\}$ such that for all $x \in \mathbb{R}^n$ a compact subspace of $\mathbb{R}^n$, the functions are identical.
\end{corollary}

\begin{proof}
\cite{He2021} proves that every piece-wise linear function on a compact subspace of real space can be represented exactly by a neural network of finite depth and width.
\end{proof}

\begin{corollary}
    For every tensor convolutional neural network (including all graph convolutional neural networks, recurrent neural networks and convolutional neural networks) with ReLU activation functions there exists a shallow neural network $\mathcal{S}$ of depth $L= 3$ with weights in the extended Reals $\bar{\mathbb{R}} = \mathbb{R} \cup \{\infty\}$ such that for all $x \in \mathbb{R}^n$, the functions are identical. 
\end{corollary}

\begin{proof}
\cite{villani2023unwrapping} show that tensor convolutional with ReLU activations can be decomposed into local linear models (analogously to the decomposition of feedforward ReLU networks).
\end{proof}

\section{Implementation} \label{sec:implementation}

Given a deep ReLU network, we propose an algorithm that finds the weights of a functionally identical shallow network. 
This algorithm is based on the constructive proof of Theorem \ref{theorem:main-shallow}. We show that every activation pattern leads to a linear program, whose feasible set is exactly a region of the partition of a ReLU network. % Some of these patterns lead to an infeasible linear program, meaning that they can never be attained by an $x \in \mathbb{R}^n$. 

In order to find the weights of the shallow network, we need to search the space of activation patterns to find all the activation patterns that yield a nonempty region. This is a vast space, with $2^{n_1 + \ldots+ n_L}$ possible patterns, which we reduce through certain heuristics. 
% Namely: 
% \begin{itemize}
%     \item If a pattern $\hat{P}^{(l)} \in \{0,1\}^{n_l}$ at layer $l$ can never be attained, 
%     %then no pattern $P= \{P^{(1)}, \ldots, P^{(L)}\}$ will include it.    
%     then no pattern $P = \{P^{(1)}, \ldots , \hat{P}^{(l)}, \ldots, P^{(L)}\}$ can be attained. 
%     \item Given $\hat{P}^{(1)}, \hat{P}^{(2)},\ldots, \hat{P}^{(l-1)}$, if $\hat{P}^{(l)}$ cannot be attained by any value $\chi^{(l)}$, then no pattern $P = \{\hat{P}^{(1)}, \ldots, \hat{P}^{(l)}, P^{(l+1)}, \ldots, P^{(L)}\}$ can be attained.  
% \end{itemize}
We develop a theory that connects linear programs to ReLU networks, and search the reduced space of patterns via a brute force algorithm.  

\subsection{Formal Correspondence between Linear Programs and Regions}

We define local and global linear programs.

\begin{definition}[Local linear program]
Let $P = \{ P^{(1)}, \ldots , P^{(L)} \}$ be an activation pattern.
The \textit{local linear program}  corresponding to $P^{(l)}$, 
is given by the set of activation vectors $\chi^{(l-1)}$ at layer $(l-1)$ such that
\[ \left(\diag(\mathbf{1} - P^{(l)})\cdot W^{(l)} - \diag(P^{(l)})\cdot W^{(l)}  \right) \cdot \chi^{(l-1)} 
\leq  - \diag(\mathbf{1}-P^{(l)})\cdot b^{(l)} + \diag(P^{(l)})\cdot b^{(l)}.\]
\end{definition}

The following lemma is used in the proof of Lemma \ref{lemma:empty-feas-set} and Proposition \ref{prop:global-lin-prog}.

\begin{lemma}\label{lemma:loc-lin-prog-n}
Let $x \in \mathbb{R}^n$, $x$ has activation pattern $P^{(l)}$ at layer $l$ only if $\chi^{(l-1)}$ satisfies the local linear program corresponding to $P^{(l)}$. \textbf{(See Appendix.)} 
% To App: \ref{app:proofs}.)}
\end{lemma}

We use the following lemma to reduce the search space of possible patterns.

\begin{lemma}\label{lemma:empty-feas-set}
Let $P = \{P^{(1)},\ldots, P^{(l)}, \ldots, P^{(L)} \}$ be the activation pattern of $\omega_P$. If the corresponding local linear program at layer $l$ has an empty feasible set, then $\omega_P = \emptyset$. \textbf{(See Appendix.)}
% To App: \ref{app:proofs}.)}
\end{lemma}

\begin{definition}[Global linear program]
Let $P = \{ P^{(1)}, \ldots , P^{(L)} \}$ be an activation pattern.
Recursively define
\begin{align*}
  A^{(1)} & := W^{(1)}  \\
  A^{(l)} & := W^{(l)} \cdot \diag (P^{(l-1)}) \cdot A^{(l-1)} \\
  d^{(1)} & :=  b^{(1)} \\
  d^{(l)} & :=  \cdot W^{(l)} \cdot \diag(P^{(l-1)}) \cdot d^{(l-1)}  + b^{(l)}.
\end{align*}
The \textit{global linear program} corresponding to $P$ at layer $l$, 
is given by the set of inputs $x\in \mathbb{R}^n$ such that for all $1\leq l \leq L$ we have 
\[ \left(\diag(\mathbf{1} - P^{(l)})\cdot A^{(l)} - \diag(P^{(l)})\cdot A^{(l)}  \right) \cdot x 
\leq  - \diag(\mathbf{1}-P^{(l)})\cdot d^{(l)} + \diag(P^{(l)})\cdot d^{(l)}.\]
\end{definition}

The following proposition is used in the algorithm to find the parameters of the hyperplanes as the constraints of the global linear program.

\begin{proposition}\label{prop:global-lin-prog}
If $x \in \mathbb{R}^n$ has activation pattern $P = \{ P^{(1)}, \ldots , P^{(L)} \}$,
then $x$ satisfies the global linear program corresponding to $P$. \textbf{(See Appendix.)}
% To App: \ref{app:proofs}.)}
\end{proposition}

\subsection{Algorithm}\label{sec:algorithm}
It is sufficient to find $H,c, \alpha, \beta$ to build the shallow network, while knowing which half spaces are needed to define each region. The algorithm we present to find the weights is structured as follows. First, we identify the set of feasible patterns. For each of these, we compute the parameters $A^{(l)}, d^{(l)} \forall l \in [L]$ of the global linear program. Stacking these matrices determines the half-space conditions for each activation pattern, and hence $-H = \texttt{stack}(\{A^{(l)}\}_{l \in [L]})$ and similarly for $c = \texttt{stack}(\{d^{(l)}\}_{l \in [L]})$. Finally, given the model weights and an activation pattern, it is easy to compute the local linear model $\alpha, \beta$ by using the explicit formula from \cite{sudjianto2020unwrapping}.   
\begin{algorithm*}
\caption{Find Shallow Network Weights}
\begin{algorithmic}[1] % The number tells LaTeX to number each line
\REQUIRE $L > 0, \forall l \in [L], n_i > 0, W^{(l)} \in \mathbb{R}^{n_l\times n_{l+1}}, b^{(l)} \in \mathbb{R}^{n_{l+1}} $ \COMMENT{this is the input}
\ENSURE $\alpha, \beta, H,c $ \COMMENT{this is the output}
\STATE{$\forall l \text{ initialise lists called }\texttt{layerwise-feasible-patterns}_l$}
\FOR{$l \in [L]$}
\FOR{$P^{(l)} \in \{0,1\}^{n_l}$}
\IF{ $\texttt{has-nonempty-local-linear-program} (P^{(l)}, W^{(l)}, b^{(l)}) = \text{True}$}
\STATE{\text{store} $P^{(l)}$ in $\texttt{layerwise-feasible-patterns}_l$}
\ENDIF
\ENDFOR
\ENDFOR
\STATE{\text{Initialise lists of lists called \texttt{feasible-patterns}, \texttt{all-hyperplanes}}}
\STATE{$\text{store } \texttt{layerwise-feasible-patterns}_1 \text{ in } \texttt{ feasible-patterns } $}
\FOR{$l \in \{2,...,L\}$}
\FOR{$P^{(l)} \text{ in } \texttt{layerwise-feasible-patterns}_l$}
\FOR{$\texttt{pattern} \text{ in } \texttt{feasible-patterns}$}
\STATE{$A^{(l)}, d^{(l)} \leftarrow \texttt{get-linear-program-weights}(P^{(l)}, \{W^{(i)}, b^{(i)}\}_{i\in[l]})$}
\IF{$\texttt{has-nonempty-global-linear-program}(P^{(l)}, \{A^{(i)}, d^{(i)}\}_{i \in [l]}) = \text{True}$}
\STATE{$\text{store } P^{(l)} \text{ in } \texttt{pattern}$}
\STATE{$\text{store } \texttt{pattern} \text{ in } \texttt{feasible-patterns}$}
\STATE{$\text{store } A^{(l)}, d^{(l)} \text{ in } \texttt{pattern}$}
\STATE{$H,c \leftarrow \texttt{get-hyperplanes}(\{A^{(i)}, d^{(i)}\}_{i \in [l]})$}
\STATE{$\text{store } H, c \text{ in } \texttt{hyperplanes}$}
\ENDIF
\ENDFOR
\ENDFOR
\ENDFOR
\FOR{$P \leftarrow \texttt{pattern} \text{ in } \texttt{feasible-patterns}$}
\STATE{$\alpha_P, \beta_P \leftarrow \texttt{get-local-linear-model}(P,\{W^{(l)},b^{(l)})\}_{l \in [L]}) $}
\STATE{store $\alpha_P, \beta_P$ in \texttt{local-linear-models}}
\ENDFOR
\RETURN \texttt{local-linear-models}, \texttt{hyperplanes}
\end{algorithmic}
\label{alg:algorithm}
\end{algorithm*}

\begin{wrapfigure}{r}{0.5\textwidth}
    % \vspace{-0.5cm}
    \includegraphics[width=0.5\textwidth]{figures/Picture 3.pdf}
    \caption{We plot the time to compute the shallow networks corresponding to randomly initialized networks $\mathcal{N}$ on the z-axis as a function of the number of neurons in the first hidden layer (y-axis) and the second hidden layer (x-axis) of $\mathcal{N}$. Error bars indicate one standard deviation.}
    \label{fig:running-time}
    \vspace{-0.5cm}
\end{wrapfigure}

While the algorithm has complexity $\mathcal{O}(2^{\Sigma_{l=1}^L n_l})$, remark that the number of activation patterns is generally small \citep{Hanin2019}, and our algorithm avoids searching the entire pattern space by pruning large portions of it.

We executed the algorithm on a local machine's CPU
% Core Intel Core i7, 
(16 GB RAM). 
We randomly initialized weights on a small network (using Xavier uniform). 
The networks have three hidden layers, with variable first and second layer width and a fixed third layer width.
We measure the time it takes to compute a shallow network for each of the randomly initialized networks.
For each combination of layer widths we repeat the experiment five times. 

The time taken to compute the algorithm for randomly initialized networks grows exponentially with the number of neurons, see Figure \ref{fig:running-time}. 
Further note that the time grows faster in the number of nodes in the second layer than in the first layer. In Figure \ref{fig:running-time}, we see that 6 neurons in the first layer, but only 5 neurons in the second layer requires slightly less than 100 seconds to compute, whereas the reverse takes slightly more than 100 seconds on average.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/Screenshot 2023-05-15 at 14.41.44.png}
%     \caption{We plot the time to compute the shallow networks corresponding to randomly initialized networks $\mathcal{N}$ on the z-axis as a function of the number of neurons in the first hidden layer (y-axis) and the second hidden layer (x-axis) of $\mathcal{N}$.}
%     \label{fig:running-time}
% \end{figure}


\section{Interpretability}\label{sec:interpretability}

The finding that any ReLU Network can be decomposed into a set of locally linear models \citep{sudjianto2020unwrapping} has made black-box neural networks more interpretable. 
More recently, an algorithm was introduced \cite{balestriero2023fast} that (like our algorithm) provides a global interpretation of the model by specifying the partition and the linear model of each part.
% Having searched all feasible patterns, we are guaranteed to have found all local linear models described by the network.

One advantage of our white-box shallow network construction is that since the network is constructed in a fully understood way it is easier to perform model surgery on it. 
% We have shown how any ReLU network can be transformed into a shallow white-box network.
% One advantage of our white-box shallow network is that since the network is constructed in a fully understood way it is easier to perform model surgery on it. 
Below, we highlight two ways in which interpretability is enhanced: 
(1) we can compute fast SHAP values for each datapoint; 
(2) given a region, we explain the region by drawing a hypercube around it.



\subsection{Calculating Exact SHAP Values}

SHAP values are popular metrics used as explanations in the field of explainable artificial intelligence \citep{lundberg2017unified}.
For a given datapoint they impute how much each input dimension contributes to the output. SHAP values are defined as follows. 

\begin{definition}[SHAP values]
\label{def:shap}
    Given a function $f\colon \mathbb{R}^n \rightarrow \mathbb{R}^m$ and an input $x\in \mathbb{R}^n$.
    A function $f_x \colon \{0,1\}^n \rightarrow \mathbb{R}^m$ is a \emph{masking function} if it evaluates $f(x)$ with $x$ unchanged when $z_i = 1$ and evaluates a `turned off' input  at dimension $i$ (such as mean or zero) when the input $z_i = 0$, for all $i \in [n]$. 
    The \emph{SHAP values} for each feature (or dimension) $i \in [n]$ are given by an  $n\times m$ matrix.
    Let $f_x \colon \{0,1\}^n \rightarrow \mathbb{R}^m$ be a masking function.
    The SHAP values are then: 
    \[\phi_i(f, x) = \sum_{z \in \{z' \in \{0,1\}^n \colon z'_i =1\} }  \frac{|z|! (n-|z| -1)!}{n!}[f_x(z) - f_x(z_{-i} )],\]
    where 
    % $\mathcal{Z} =\{z \in \{0,1\}^n \colon z_i =1\} $ and  
    $(z_{-i})_j := z_j$ for all $j$ excluding $i$; and $|z|$ counts the number of nonzero entries of $z$. 
\end{definition}

Typically, for machine learning models, these SHAP values are estimated. 
However, for a linear model they are known \citep{lundberg2017unified} and are given in terms of the mean of a distribution over the input space.
Hence, given a decomposition of a network we can give exact SHAP values.
% $\mathcal{N}$ into local linear models, we can give exact SHAP values $\phi_i(\mathcal{N}, x)$.
% Given a decomposition of a network $\mathcal{N} \colon \mathbb{R}^n \rightarrow \mathbb{R}^m$
% into $p$ local linear models $f_i(x) = \alpha_i x + \beta_i$, 
% the number of input dimensions and thus the number of SHAP values for the network is $n$.


\begin{proposition}
Let $\mathcal{N} \colon \mathbb{R}^n \rightarrow \mathbb{R}^m$ be a ReLU network with decomposition into local linear models. Let $\omega$ be a region with local linear model $f(x') = \alpha x' + \beta$, let $D$ be a distribution over $\omega$ and let $x \in \omega$. Let $f_x$ be a masking function, where given a masked dimension 
% (i.e. an entry for which $f_x$ is not specified) 
we define $f_x$ as returning a sample from the distribution $D$. Then the SHAP values for feature $i$ are given by 
\[ \phi_i(\mathcal{N}, x) = \alpha ( x - \mathbb{E}_{D(\omega)}(x)).\]
\end{proposition}


\begin{proof}
Since $\mathcal{N}$ is linear on the polytope $\omega$, for every sampled input $X \sim D(\omega)$ we will have that  $\mathcal{N}(X) = f_x(X) = \alpha X + \beta$. The result then follows from  \cite{lundberg2017unified}. 
\end{proof}

A consequence of this proposition is that SHAP values can be computed exactly and almost instantly from the decomposition after computing the mean of the background distribution. \footnote{This can be done analytically if we choose the distribution to be uniform. However, it may be inappropriate to select this distribution, since the polytope may not be bounded.}

% [CITE MATTIA] shows the explicit SHAP values can be given for  features of the network $\mathcal{N}$ [CITE MATTIA] the authors discuss how we can use the decomposition to find explicit SHAP values, whenever we assume that the background distribution is defined on the region in which $x$ belongs to. 



\subsection{Explainability via Hypercubes around Regions}

Given a region, we can explain it by drawing the smallest possible hypercube around it. This enables us to approximately describe, using a small number of parameters: the region, the location of the region and the largest bounds in terms of the input features. In particular, we highlight a tension between faithfully representing the region, which would require specifing many hyperplanes and $n$ parameters for each one of these hyperplanes. 

We trained a feedforward ReLU network with neuron vector [5,7,4] on the first two dimensions of the Iris dataset \citep{iris-dataset} for 5000 epochs with a Sigmoid output layer, cross entropy loss and Adam with learning rate 0.0001 and betas equal to 0.9 and  0.999.
We then used our algorithm, as introduced in Section \ref{sec:algorithm} to decompose the neural network and find all regions. We then select the regions where test data lives and record them in Figure \ref{fig:plot-regions}. 
\begin{figure}[h]
    \vspace{-0.3cm}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/Picture 2.pdf}
    \vspace{-0.5cm}
    \caption{We plot the regions (in green) for a test portion (40\%) of the first two dimensions of the Iris dataset. 
    % \footnote{We chose a two-dimensional input space to visualize hypercubes}. 
    All these datapoints (red crosses) fall in one of five regions. In red we draw the smallest hypercube that fits the entire region. 
    The x-axis represents petal length, and the y-axis petal width. }
    \label{fig:plot-regions}
    \vspace{-0.2cm}
\end{figure}
The hypercubes are coarse explanations that become less faithful as the number of dimensions increases. 
% The hypercube explains a region by, in each dimension, giving a minimum and maximum value of the region.
However, identifying the position 
as well as inspecting the inputs are in a region helps us identify common characteristics of the inputs; 
the size parameter of the cube is to be used relatively to others in order to capture an approximation of the size of the region.

\subsection{Unique Representation of Function}

Given two ReLU networks it is easy to verify that they coincide or diverge on a specific dataset. 
However, if that they do coincide it is non-trivial to find out if they encode the same function (on the entire space of possible inputs).
Our algorithm converts any representation of the same function to the same shallow network.
The shallow network representation is unique because the weights encoding the linear models are lexicographically ordered, as are the half-space conditions.

Our construction of a shallow network is not injective, in that multiple (functionally identical) deep networks with different architectures can all map to the same shallow network. 
If we consider equivalence classes of neural networks that each encode a different function, then our shallow networks can be seen as a representative of their equivalence class. 

\section{Discussion}

% summary of our findings

% % The significance of the result reaches beyond interpretability, providing insight on the nature of deep learning systems as representation machines. 
% Deep neural networks tend to learn hierarchical concepts, with later layers containing more complex concepts than early layers \cite{}.
% We provide insight on the nature of deep learning as representation machines, by our finding that these concepts can be rearranged in a horizontal fashion, while preserving their functionality. 
% % For example, \cite{----} notice the emergence of complex concepts in later layers of a neural network; the fact that we can preserve the semantic content of the network with fewer layers seems to work in analogy to how we can [... explain something complex in many words].

Our contribution has been to prove all deep ReLU networks can be rewritten as a shallow network (Theorem \ref{theorem:main-shallow}), while providing a way to compute the weights algorithmically (Algorithm \ref{alg:algorithm}). 
This enhances interpretability by allowing us to quickly compute feature importance and giving  details of the exact, local functional relationship between input and output.
Deep neural networks discern hierarchical concepts, with later layers encapsulating more complex concepts than earlier ones. 
Remarkably, we demonstrate that these concepts can be rearranged horizontally, maintaining their original functionality. 
This restructuring allows us to derive a shallow network from a deep one.


% Deep neural networks discern hierarchical concepts, with later layers encapsulating more complex concepts than the earlier ones. Remarkably, we demonstrate that these concepts can be rearranged horizontally, maintaining their original functionality. This restructuring process allows us to derive a shallow network from a deep one, creating a non-injective map between functionally identical deep networks of varying architectures and a single shallow network. The shallow networks can thus serve as representatives of the equivalence classes of neural networks, each encoding a unique function. 
% CHAT GPT 

% Future work ideas
% We hope to expand this work to attention layers.
% Proving minimum bounds on functionally identical networks, with and without weights in the extended Reals.


\subsection{Limitations}

The construction of a shallow network makes use of infinite weights.
Although these weights can be implemented in \texttt{Python}, they can not be fine-tuned using gradient descent. 
Note that the weights encoding the linear models can be fine-tuned. 
If one wanted to fine-tune the linear models, while keeping the transparent network structure, then the weights encoding identity matrices between the blue blocks in Figure \ref{fig:schematic-rep-of-proof} should be frozen. 
Additionally, the four weight matrices denoted by $\alpha$ and $-\alpha$ between the blue and green blocks should be updated in conjunction with one another.  
% The weights encoding the local linear models can be fine-tuned. Not all weights can be updated via gradient descent, since some of them are \texttt{inf}. In particular, the weights that are used to form a region indicator function, can not be fine-tuned.

The current algorithm is well suited for small models, but large computational resources are needed to perform the search of feasible patterns in larger models. Future work should focus on finding efficient heuristics to prune the space of possible activation patterns. Moreover, research should prioritise developing faithful explanations that navigate the complexity of these models.

%Although our algorithm proves effective for smaller models, it requires substantial computational resources for larger models due to the extensive search of feasible patterns. Therefore, future work should concentrate on developing efficient heuristics to prune the space of possible activation patterns. It is important to note that while we have made strides in making neural networks more interpretable, providing concise explanations remains a complex endeavor.

==> old-proof.tex <==
\begin{lemma}
\begin{align*} 
& ReLU \left( \left(\diag(\mathbf{1} - P^{(n)})\cdot W^{(n)} + \diag(P^{(n)})\cdot W^{(n)}  \right) \cdot \chi^{(n-1)} 
+  \diag(\mathbf{1}-P^{(n)})\cdot b^{(n)} + \diag(P^{(n)})\cdot b^{(n)} \right) \\
& = 
ReLU 
\left(
\diag(P^{(n)})\cdot W^{(n)} \cdot \chi^{(n-1)} +
\diag(P^{(n)})\cdot b^{(n)}.
\right) 
\end{align*}
\end{lemma}

\begin{proof}
If $P^{(n)}_i = 0$
then $( W^{(n)} \chi^{(n-1)} + b^{(n)} )_i \leq 0$,
so 
\[\diag(\mathbf{1} - P^{(n)})\cdot W^{(n)}  \cdot \chi^{(n-1)} 
+ \diag(\mathbf{1}-P^{(n)})\cdot b^{(n)} \leq 0.\]
If $P^{(n)}_i = 1$
then $( W^{(n)} \chi^{(n-1)} + b^{(n)} )_i > 0$,
so
\[ \diag(P^{(n)})\cdot W^{(n)} \cdot \chi^{(n-1)} + \diag(P^{(n)})\cdot b^{(n)} > 0.\]
\end{proof}

Main theorem.

\begin{proof}

Our strategy will be to build a first layer that encodes the linear models and the half-spaces that span the partition. 
We will use the weights that encode the half-spaces to, in the last layer, select the correct linear model out of the list of linear models. 

Without loss of generality, we assume that $\mathcal{N}: \mathbb{R}^n \rightarrow \mathbb{R}$, i.e. we assume $m=1$. If the dimension of the output space $m >1$, then we repeat the construction of the last layer $m$ times. Let $(\{f_\omega\}_{\omega \in \Omega}, \Omega)$ be the decomposition that corresponds to $\mathcal{N}$. Label the parts $1,...,p$.

Let $\Lambda$ be a linear transformation given by: 
\[
\Lambda(x) = \alpha^T x + \beta,
\]
where $\alpha, \beta$ are respectively a $p \times n$ matrix and a $p$-dimensional bias, such that the row $\alpha_i$ and entry $\beta_i$ contain the coefficients of $f_i$. Note that, in this step, if $m > 1$, then the matrix and vector would be $p \cdot m \times n$ and $p \cdot m$ dimensional respectively.

Each part is a polytope and we can represent it as the intersection of half-spaces \citep{sudjianto2020unwrapping}. In particular, let $H_1,...,H_k$ be the set of half-spaces that generate the partition, where each $H_i$ is given by the set of all $x \in \mathbb{R}^n$ such that: 
\[ h_{i,1} h_1 + h_{i,2} x_2 + ... + h_{i,n} x_n  > c_i.\]
Let $\Psi$ be a linear transformation applying all the half-space conditions: 
\begin{align*}
    \Psi(x) = H x + c 
    = \begin{bmatrix} -h_{1,1} & -h_{1,2} & ... & -h_{1,n} \\ -h_{2,1} & -h_{2,2} & ... & -h_{2,n}\\ ... & & & ... \\  - h_{k,1} & - h_{k,2} & ... & - h_{k,n} \end{bmatrix} \begin{bmatrix} x_1 \\ x_2 \\... \\ x_n \end{bmatrix}+ \begin{bmatrix} c_1 \\ c_2\\  ... \\ c_k \end{bmatrix}, 
\end{align*}
where $H$ is a $2k \times n$ matrix. 
Entry-wise this matrix $\Psi(x)$ looks as follows
\[\Psi(x)_{i} = - h_{i,1} \cdot x_1 - h_{i,2} \cdot x_2 -  ... - h_{i,n} \cdot x_n + c_{i}.\] 
% Notice that this implies that $ReLU(B(x))$ has a positive entry at $2i-1$ only if $x\in H_i$, and $ReLU(B(x))_{2i} = 0 $ whenever $x \in H_i$. 
Notice that this implies that whenever $x\in H_i$ we have $ReLU(\Psi(x))_{i} = 0$. 
The \textbf{first layer} is given by: 
\[
\chi^{(1)} = \text{ReLU}( W^{(1)}x +b^{(1)})  =\text{ReLU} \left(\begin{bmatrix}
    \alpha \\
    - \alpha \\
    H \\ H
\end{bmatrix} x + \begin{bmatrix} \beta \\ -\beta \\ c \\ c \end{bmatrix} \right),
\]
which is an activation vector of length $2\cdot p\cdot m + 2 \cdot k$.

This transformation develops the building blocks to generate neurons that are only inactive when $x$ is in a certain region. In particular, we want to construct a layer that only has an inactive neuron whenever the input in a particular region. 
In other words, we find a $p \times k$ zero-one matrix $R$ which describes the regions in terms of which boundaries are active. Precisely, we can design $R$ so that $R \cdot \text{ReLU}(\Psi(x))$ has a zero entry at $j$ only when $x \in \mathbb{\omega}_j, j \in \{1,...,p\}$. 
Assume without loss of generality that the  half-space conditions corresponding to region $\omega_j$ are $H_1, \ldots , H_a$ be the . The half-space conditions $H_1, \ldots , H_a$ are satisfied at a point $x$ if and only if $x \in \omega_j$.
We construct $R$ such that at row $j$ it assigns a 1 to entries $1, \ldots, a$, and a 0 to all other entries in that row.  
This leads to the description of the \textbf{second layer}: 
\begin{align*}
\chi^{(2)} 
= \text{ReLU}( W^{(2)} \chi^{(1)} + b^{(2)}) 
&= \text{ReLU} 
\left(\begin{bmatrix} 
I_{p} &  &  & 0 \\ 
 & I_{p} &  &  \\
 &  & R & \\ 
0 &  &  & R \end{bmatrix} \chi^{(1)} + \begin{bmatrix}
    0 \\  \\  \\ 0
\end{bmatrix} \right) \\
& = \text{ReLU} \left(\begin{bmatrix} \hspace{12pt} ReLU( \Lambda(x) )  \\
\hspace{12pt} ReLU( - \Lambda(x) ) \\
R \cdot ReLU(\Psi(x))  \\
R \cdot ReLU(\Psi(x)) \end{bmatrix} \right), 
\end{align*}
as an activation vector of length $4 \cdot p \cdot m$.
 
Finally, the third layer requires constructing a matrix $ O_{2p} = \theta \cdot I_{2p}$, that multiplies all non-zero values of $R \cdot \text{ReLU}(\Psi(x))$ by an arbitrarily large real number $\theta \in \mathbb{R}$, such that if we subtract this matrix from the linear values we get a vector
\[\Lambda(x) - O_p \cdot \text{ReLU} (R \cdot \text{ReLU}(\Psi(x))) 
= \begin{bmatrix} - \theta \\ \vdots \\ -\theta \\\Lambda(x)_j \\ - \theta \\ \vdots \\ - \theta \end{bmatrix},\] 
of length $p$ for which the only positive entry is given by the linear model at the region $j$ evaluated at $x$. Since each $R\cdot \text{ReLU} (\Psi(x))$ can be arbitrarily small, we must choose $ \theta = \infty$, such that $\infty \cdot 0 = 0$ and $\infty \cdot a = \infty$ for all $|a| >0, a \in \mathbb{R}$.
Note that Python contains such a constant, denoted by \texttt{inf}. 
This entails our \textbf{third layer} activations are given by:   
\begin{align*}
\chi^{(3)} 
= 
\text{ReLU}(W^{(3)} \chi^{(2)} + b^{(3)}) 
& = \text{ReLU} \left(\begin{bmatrix} I_{2p}  & - O_{2p}  \end{bmatrix} \chi^{(2)} \right) \\
& = \text{ReLU} \left( \begin{bmatrix} I_{2p}  & - O_{2p}  \end{bmatrix} \begin{bmatrix} \hspace{12pt} ReLU( \Lambda(x) ) \\ \hspace{12pt} ReLU( - \Lambda(x) )\\ R \cdot ReLU(\Psi(x)) \\ R \cdot ReLU(\Psi(x)) \end{bmatrix} \right) \\
& = \text{ReLU} \left( \begin{bmatrix} \hspace{3.5pt} ReLU( \Lambda(x) ) \hspace{4pt} - O_{p} \cdot R \cdot ReLU(\Psi(x)) \\ ReLU( - \Lambda(x) ) - O_{p} \cdot R \cdot ReLU(\Psi(x)) \end{bmatrix} \right)
\end{align*}
which is a vector of length $2p$ with exactly one non-zero entry at either $j$ or $2j$. This non-zero entry is $L(x)$ at row $j$ (if $L(x)$ is positive) or $-L(x)$ at row $2j$ (if $L(x)$ is negative).

Lastly we need a layer to project onto $\mathbb{R}^m$. This projection requires $2p$ weights since we assumed $m=1$. When we project the $-L(x)$ value to the output layer, we need to swap the sign. The first $p$ weights of $W^{(4)}$ are 1 and the last $p$ weights are $-1$.
\end{proof}


==> old-shap.tex <==
\begin{definition}[\textbf{SHAP Values}]
    Given a function $f \colon \mathbb{R}^n \rightarrow \mathbb{R}^m$, the SHAP values for feature $i \in [n]$ are given by:
    \[\phi_v(i) = \sum_{S \in \mathcal{P}([n]) / \{i\} } \frac{(N-|S| +1)|S|!}{N!} \Delta_v(S,i),\]
    where $\mathcal{P}([n])$ is the set of a all subsets of $[n]$, $v:\mathcal{P}([n]) \rightarrow \mathbb{R}$ is a value function, and $\Delta_v(S,i)$ is the marginal contribution of a feature $i$ on a subset $S \in \mathcal{P}([n])$, which we refer to as a \textit{coalition} of features, is given by: 
    \[\Delta_v (i,S) = v(\{i\} \cup S) - v(S).\]
\end{definition}

\begin{definition}
    Let $f\colon \mathbb{R}^n \rightarrow \mathbb{R}^m$, be an arbitrary function and $h_x: \{0,1\} \rightarrow \mathbb{R}^n$ be a masking function such that $f \circ h_x = f_x \colon \{0,1\}^n \rightarrow \mathbb{R}^m$ is a mapping that returns a \textit{turned off} value (such as mean or zero) when $z_i = 0$ and keeps the value of $x$ unchanged when $z_i = 1$, for all $i \in [n]$. The SHAP values $\phi_i:[\mathbb{R}^n, \mathbb{R}^m] \times \mathbb{R}^n \rightarrow \mathbb{R}^m$ for feature $i \in [n]$ at point $x\in \mathbb{R}^n$ are given by: 
    \[\phi_i(f, x) = \sum_{z \in \mathcal{Z}} \frac{|z|! (n-|z| -1)!}{n!}[f_x(z) - f_x(z_{-i} )],\]
    where $\mathcal{Z} =\{z \in \{0,1\}^n \colon z_i =1\} $ and  $(z_{-i})_j = z_j$ for all $j$ excluding $i$; $|z|$ counts the number of nonzero entries of $z$.  
\end{definition}

\begin{definition}[SHAP values] \label{def:shap}
    Given a function $f\colon \mathbb{R}^n \rightarrow \mathbb{R}^m$ and an input $x\in \mathbb{R}^n$, the SHAP values for each feature (or dimension), $i \in [n]$ are given by an  $n\times m$ matrix.
    Consider the function $f_x \colon \{0,1\}^n \rightarrow \mathbb{R}^m$ which returns a \textit{turned off} value (such as mean or zero) when the input $z_i = 0$ and keeps the value of $x$ unchanged when $z_i = 1$, for all $i \in [n]$. 
    The SHAP values are then: 
    \[\phi_i(f, x) = \sum_{z \in \{z' \in \{0,1\}^n \colon z'_i =1\} }  \frac{|z|! (n-|z| -1)!}{n!}[f_x(z) - f_x(z_{-i} )],\]
    where 
    % $\mathcal{Z} =\{z \in \{0,1\}^n \colon z_i =1\} $ and  
    $(z_{-i})_j := z_j$ for all $j$ excluding $i$; and $|z|$ counts the number of nonzero entries of $z$. 
\end{definition}

\begin{proposition}
Given a ReLU network $\mathcal{N}:\mathbb{R}^n \rightarrow \mathbb{R}^m$ with decomposition into local linear models. Let $\omega$ be a region with local linear model $f(x') = \alpha x' + \beta$, and let $x \in \omega$. Moreover, let $f_x$ be a function of type  Definition \ref{def:shap}, which given a masked dimension (i.e. an entry for which $f_x$ is not specified) returns a sample from a background distribution $D(\omega)$ over $\omega$. Then the SHAP values for feature $i$ are given by 
\[ \phi_i(\mathcal{N}, x) = \alpha ( x - \mathbb{E}_{D(\omega)}(x)).\]
\end{proposition}

\begin{definition}[Masking function]
    Given a function $f\colon \mathbb{R}^n \rightarrow \mathbb{R}^m$ and an input $x\in \mathbb{R}^n$.
    A function $f_x \colon \{0,1\}^n \rightarrow \mathbb{R}^m$ is a masking function if it evaluates $f(x)$ with $x$ unchanged when $z_i = 1$ and evaluates a `turned off' input  at dimension $i$ (such as mean or zero) when the input $z_i = 0$, for all $i \in [n]$. 
\end{definition}

\begin{definition}[SHAP values] \label{def:shap}
    Given a function $f\colon \mathbb{R}^n \rightarrow \mathbb{R}^m$ and an input $x\in \mathbb{R}^n$, the SHAP values for each feature (or dimension), $i \in [n]$ are given by an  $n\times m$ matrix.
    Let $f_x \colon \{0,1\}^n \rightarrow \mathbb{R}^m$ be a masking function.
    The SHAP values are then: 
    \[\phi_i(f, x) = \sum_{z \in \{z' \in \{0,1\}^n \colon z'_i =1\} }  \frac{|z|! (n-|z| -1)!}{n!}[f_x(z) - f_x(z_{-i} )],\]
    where 
    % $\mathcal{Z} =\{z \in \{0,1\}^n \colon z_i =1\} $ and  
    $(z_{-i})_j := z_j$ for all $j$ excluding $i$; and $|z|$ counts the number of nonzero entries of $z$. 
\end{definition}
